Suppressing unwanted fluctuations in QAOA and approximate quantum annealing

The quantum approximate optimisation algorithm (QAOA) was partially inspired by digitising quantum annealing. Based on this inspiration, we develop techniques to use the additional flexibility of a universal gate-model quantum computer to mitigate fluctuation effects which are known to distort the search space within quantum annealing and lead to false minima. We find that even just the added ability to take Pauli X measurements allows us to modify the mixer angles to counteract these effects by scaling mixer terms in a way proportional to the diagonal elements of the Fubini-Study metric. We find that mitigating these effects can lead to higher success probabilities in cases where the energy landscape is distorted and that we can use the same Pauli X measurements to target which variables are likely to be susceptible to strong fluctuations. The effects of the methods we introduce are relevant even at relatively low depth of $p=10-20$, suggesting that the techniques we are developing are likely to be relevant in the near term. Furthermore, since these methods rely on controlling a degree of freedom which is not typically modified in QAOA, our methods will be compatible with a wide range of other QAOA innovations. We further verify that these fluctuation effects can be observed on an IonQ Harmony QPU.

==> SpecializedRandomQUBOs.tex <==
%% Creating this subsection to include the random plots for the QUBOs generated from the algorithm
Unable to think of a better title to this section. Please feel free to rename it.

\begin{figure*}[htp!]
\begin{subfigure}[b]{0.5\textwidth}
	\begin{centering}
	\includegraphics[width=1\textwidth]{CDF_figs/p10_runs25.png}
	\par
	\end{centering}
	\caption{p = 10}
	%\label{fig:433_varying_p10}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
	\begin{centering}
	\includegraphics[width=1\textwidth]{CDF_figs/p30_runs25.png}
	\par
	\end{centering}
	\caption{p = 30}
	%\label{fig:433_varying_p30}
\end{subfigure}\\[1ex]
\begin{subfigure}[b]{\textwidth}
\centering
	\begin{centering}
	\includegraphics[width=0.5\textwidth]{CDF_figs/p50runs25.png}
	\par
	\end{centering}
	\caption{p  = 50}
	%\label{fig:433_varying_p50}
\end{subfigure}
\caption{CDF (fraction of runs) of success probability at the end of AQA solving a 10 variable problem generated using algorithm \ref{Alg:problem_generation} with $n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$, $J_{gadget}=0.25$, $J_{\mathrm{couple}}=0.5$, $\mathrm{Bias}=1.5$ for (a) p = 10, (b) p = 30, and (c) p = 50.  Blue corresponds to an unmodified mixer, while gold corresponds to the suppressed mixer and green to a thresholded mixer}
\end{figure*}

In this section, we further elaborate on the performance of the suppressed and thresholded mizers for the QUBOs generated using algorithm \ref{Alg:problem_generation}. In particular, observe the following behaviour.

% \begin{figure}
% \begin{centering}
% \includegraphics[width=13cm]{merged_figure.png}
% \par
% \end{centering}
% \label{fig:433_varying_p}
% \caption{CDF (fraction of runs) of success probability at the end of AQA solving a 10 variable problem generated using algorithm \ref{Alg:problem_generation} with $n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$, $J_{gadget}=0.25$, $J_{\mathrm{couple}}=0.5$, $\mathrm{Bias}=1.5$ for (a) p = 10, (b) p = 30, and (c) p = 50.  Blue corresponds to an unmodified mixer, while gold corresponds to the suppressed mixer and green to a thresholded mixer}
% \end{figure}



Firstly, we generate different random realizations of ten variable QUBO with $n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$, $J_{gadget}=0.25$, $J_{\mathrm{couple}}=0.5$, $\mathrm{Bias}=1.5$, and compute the success probability by applying AQA with the three different mixer strategies, namely the unmodified mixer, the suppressed mixer, and the thresholded mixer,  to each of these QUBOs. Figures \ref{fig:433_varying_p10}, \ref{fig:433_varying_p30}, and \ref{fig:433_varying_p50} show the empirical CDF plots of the success probabilities obtained using the three different strategies for three different values of $p$ for 25 randomly generated QUBOs. The plots confirm the trend observed earlier for a single sample (see figures \ref{fig:gad_1_p_1_4_success} \ref{fig:gad_1_p_1_4_false}), on a random collection of QUBOs, where the thresholded and suppressed techniques both significantly outperform an unmodified mixer, with the thresholded technique performing the best, and a general upward trend in success probability with increasing p.

\begin{figure*}[htp!]
\begin{subfigure}[b]{0.5\textwidth}
	\begin{centering}
	\includegraphics[width=1\textwidth]{CDF_figs/size211_p50_runs25.png}
	\par
	\end{centering}
	\caption{$n_\mathrm{cut}=2$, $n_\mathrm{gadget}=1$}
	\label{fig:size211_p50_runs25}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
	\begin{centering}
	\includegraphics[width=1\textwidth]{CDF_figs/size333_p50_runs25.png}
	\par
	\end{centering}
	\caption{$n_\mathrm{cut}=3$, $n_\mathrm{gadget}=3$}
	\label{fig:size333_p50_runs25}
\end{subfigure}\\[1ex]
\begin{subfigure}[b]{\textwidth}
	\begin{centering}
	\includegraphics[width=0.5\textwidth]{CDF_figs/p50runs25.png}
	\par
	\end{centering}
	\caption{$n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$}
	\label{fig:size433_p50_runs25}
\end{subfigure}
\caption{CDF (fraction of runs) of success probability at the end of AQA solving a 10 variable problem generated using algorithm \ref{Alg:problem_generation} with  $J_{gadget}=0.25$, $J_{\mathrm{couple}}=0.5$, $\mathrm{Bias}=1.5$ and (a) $n_\mathrm{cut}=2$, $n_\mathrm{gadget}=1$,, (b) $n_\mathrm{cut}=3$, $n_\mathrm{gadget}=3$, and (c) $n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$,  Blue corresponds to an unmodified mixer, while gold corresponds to the suppressed mixer and green to a thresholded mixer}
\end{figure*}

Secondly, to study how the performance of the three methods scale with the size of the QUBOs, we randomly generate 25 QUBOs for each of the following three sizes: (a) four with $n_\mathrm{cut}=2$, $n_\mathrm{gadget}=1$, (b) nine with $n_\mathrm{cut}=3$, $n_\mathrm{gadget}=3$, and (c) ten with $n_\mathrm{cut}=4$, $n_\mathrm{gadget}=3$. Figures \ref{fig:size211_p50_runs25}, \ref{fig:size333_p50_runs25} and \ref{fig:size433_p50_runs25} demonstrate the CDF plots of success probabilities at the end of applying the AQA with the three mixer strategies, using $p=50$. We observe that as the size of the QUBO increases, the advantage shown by the suppressed and thresholded schemes over the unmodified technique increases, which shows a useful trend needed as the QUBOs are scaled in size.




